Social learning via actions in bandit environments

I study a game of strategic exploration with private payoffs and public actions in a Bayesian bandit setting. In particular, I look at cascade equilibria, in which agents switch over time from the risky action to the riskless action only when they become sufficiently pessimistic. I show that these equilibria exist under some conditions and establish their salient properties. Individual exploration in these equilibria can be more or less than the single-agent level depending on whether the agents start out with a common prior or not, but the most optimistic agent always underexplores. I also show that allowing the agents to write enforceable ex-ante contracts will lead to the most ex-ante optimistic agent to buy all payoff streams, providing an explanation to the buying out of smaller start-ups by more established firms.

==> notes.tex <==
\section{After Dec 2 presentation}

\begin{itemize}
    \item Entire structure of the paper and its results seem to hinge on the specific reward process - one success reveals the state. There will be questions later about this.
    \item There seem to be implicit assumptions about the refinement being used. What excludes strategies that have punishments on path? Or do they not need to be excluded?
    \item Huge problem with mixed strategy equilibria, especially when agents may be indifferent between the arms or when they mix on path just to slow information revelation. Then, cutoffs themselves can be random.
    \item What do cascades actually look like? Understanding the cutoffs better.
    \item Agents coordinating - can coordination improve exploration (maybe a correlation device)? Can agents explore more than socially optimum?
    \item We assume common knowledge of strategies here, but this may be impractical for large $n$. It may be that agents also have to learn others' strategies.
\end{itemize}
